From Self-Attention to Markov Models: Unveiling the Dynamics of Generative Transformers

Modern language models rely on the transformer architecture and attention mechanism to perform language understanding and text generation. In this work, we study learning a 1-layer self-attention model from a set of prompts and associated output data sampled from the model. We first establish a precise mapping between the self-attention mechanism and Markov models: Inputting a prompt to the model samples the output token according to a context-conditioned Markov chain (CCMC) which weights the transition matrix of a base Markov chain. Additionally, incorporating positional encoding results in position-dependent scaling of the transition probabilities. Building on this formalism, we develop identifiability/coverage conditions for the prompt distribution that guarantee consistent estimation and establish sample complexity guarantees under IID samples. Finally, we study the problem of learning from a single output trajectory generated from an initial prompt. We characterize an intriguing winner-takes-all phenomenon where the generative process implemented by self-attention collapses into sampling a limited subset of tokens due to its non-mixing nature. This provides a mathematical explanation to the tendency of modern LLMs to generate repetitive text. In summary, the equivalence to CCMC provides a simple but powerful framework to study self-attention and its properties.

==> sec/MainQuestions.tex <==
\section{Main Questions}
\textbf{Setting 1: Position Encoding-free.} Let $\Pb\in\R^{K\times K}$ be a Markov chain probability transition where each column add up to 1. Let $\Sb_1=[2,3,\dots,K,1]$ and $\Sb_k=[k+1,k+2,\dots,K,1,2,\dots,k]$ be the sequence obtained by shifting $\Sb_1$ by $K-1$ entries to the left.

\textbf{Ground-truth attention model.} Ground-truth model outputs the next token based on $\Pb$ transitions. Namely, if we input $\Sb_k$ with the last token, ground truth outputs other tokens with probabilities $\pb_{k}$ where $\pb_k$ is the $k$'th column.

\begin{itemize}
\item If the input sequence $X$, the transitions are given by $\Pb_X=\text{column\_adjust}(\text{FreqX}\odot \Pb)$.
\item \textbf{Question 1: Multiple IID trajectories.} Generate $N$ sequences of length $T$. Each sequence samples token embeddings IID according to a distribution $q\in\R^K$. In the simplest case, $q$ is uniform distribution i.e.~$q_k=1/K$. We observe these sequences and their next token. Our goal is to learn $P$ by training an attention model. Simply estimate one column i.e.~estimate a discrete $K$ valued distribution based on samples of its $T$-wise restrictions.
\item \textbf{Question 2: Single trajectory.} Start from trajectory $\Sb_1$ and observe it for a duration of $N$. Our goal is to learn $P$ by training an attention model.
\begin{itemize}
\item \textbf{Question 2 variation: Multiple trajectories from each token.} Observe $K$ trajectories starting from $\Sb_1,\dots,\Sb_K$.
\end{itemize}
\item Note that, since theory setting is convex, training an attention model will likely be perfectly identical to fitting a $-log$ loss to Markov chain transitions.
\item Number one consideration: 
\begin{itemize}
    \item Q1: Whether estimation is unbiased: Whether the optimal $P^*$ is the underlying Markov chain
    \item Q2: Whether attention optimization is equivalent to a discrete $P$ fit
    \begin{align}
    &\Pb^*=\arg\min_{\Pb} -\E_{X\sim\Dc}[\log_{\text{FreqX}\odot \Pb}(x_{next}|X_{last})]\tag{PopRisk}\\
    &\hat{\Pb}=\arg\min_{\Pb} -\frac{1}{N}\sum_{i=1}^N\log_{\text{FreqX}\odot \Pb}(x_{next}|X_{last})\tag{EmpRisk}\\
    \end{align}
\end{itemize}
\item Key consideration: Sample complexity analysis should capture: (1) Complexity of the Markov chain. (2) Coverage i.e. if you have short IID trajectories, they should better cover all transitions.
\item Single trajectory might not generalize due to \emph{collapse/degeneration/singleton} issues
\begin{itemize}
\item Claim: $\pi=\text{diag}(\pi)\Pb\pi\implies c\cdot[\text{zero-one vector}] =\Pb\pi$. Only stable solution under mild conditions is vectors with single one? $\pi_{next}\gets P\pi_{cur}$, $\pi_{next}\gets \text{diag}(\pi_{\text{cur}}) P\pi_{cur}$
\end{itemize}
\end{itemize}

==> sec/equivalency.tex <==
\section{Equivalency of CA and PCMC Models}\label{sect equivalency}
In this section, we establish an invertible map from the cross-attention model to the prompt-conditioned Markov chain model. This mapping is critical while identifying the conditions that guarantee consistent estimation.



\begin{definition}
    
\end{definition}



\begin{lemma}\label{lemma equivalence minimizer}
    Let $(\X_i, y_i)_{i=1}^n$ be an arbitrary training set. Let $\hat{\W}$ and $\hat{\Pb}$ be the solutions of empirical risk minimization problems under the self-attention model and the prompt-conditioned Markov chain model, respectively. Then, we have \begin{align}
        \hat{\Pb} = \bold{PCMC}(\hat{\W})    \end{align}Furthermore, let's consider $\hat{\W}$ and $\hat{\Pb}$ as random variables of $\Dc_{\Xc}$ and $\W^{grd}$. Then, we have
    \begin{align}
        \Lc(\hat{\W}) - \Lc(\W^*) = \sum_{{k=1}}^K p_k D_{KL}( \bpi_k^* || \hat{\bpi}_{k})
    \end{align}
    where $p_k$ is the weights of mixture distribution $\Dc_{\Xc}$ and $D_{KL}( \bpi_k^* || \hat{\bpi}_{k})$ represents the KL-divergence between the $k^{\text{th}}$ rows of $\Pb^*$ and $\hat{\Pb}$.
\end{lemma}
Lemma \ref{lemma equivalence minimizer} provides a playground to study the excess loss of $\Lc(\hat{\W}) - \Lc(\W^*)$ without delving deep into the self-attention model. Thanks to this playground, we analyze the excess loss by the prompt-conditioned Markov chain model throughout the paper.  


==> sec/lowrank.tex <==
\newpage
\section{Learning $\Pb^{grd}$ with Low Rank $\W$ }
\begin{theorem}
    Suppose the self-attention problem is low-rank  $\text{rank}(\W) = m < d$  
\end{theorem}
\begin{definition}[Subspace (Revised)]
        
\end{definition}
\begin{definition}[Independence (Revised)]
    A set of probability vectors $\{\bpi_k\}_{k=1}^K \in \R^K$ are independent if the vector equation
    \begin{align}
        (\bpi_1)^{q_1} \odot (\bpi_2)^{q_2} \odot \dots \odot (\bpi_{K-1})^{q_{K-1}} = q_k \bpi_{K}
    \end{align}
    has no solution for $\{q_k\}_{k=1}^K \in \R$. 
\end{definition}
\begin{definition}[Rank(Revised)]
    
\end{definition}
